Aren't we all nearest neighbors: Spatial trees, high dimensional reductions and batch nearest neighbor search

We start with a review of the pervasiveness of the nearest neighbor search problem and techniques used to solve it along with some experimental results. In the second chapter, we show reductions between two different classes of geo- metric proximity problems: the nearest neighbor problems to solve the Euclidean minimum spanning tree problem and the farthest neighbor problems to solve the k-centers problem. In the third chapter, we unify spatial partitioning trees un- der one framework the meta-tree. Finally, we propose a dual tree algorithm for Bichromatic Closest Pair and measure the complexity of batch nearest neighbor search.

==> experimental.tex <==
The above highlights the power randomness affords us in reasoning about the proximity of points in Euclidean space we summarize these effects below.

\begin{enumerate}
\item Random Projection as a dimensionality reduction preprocessing step via the Johnson-Lindenstrauss Lemma
\item Random Partition of space via Rp Trees
\item Randomness over size of spill
\item Randomness over datastructure via Random Forests
\end{enumerate}
The first point can be understood from \cite{DG02}, the second and third from \cite{DS14}. The fourth introduces some complexity: In fact Rp-Trees only have two hyperparameters to tune, the maximum allowed depth of the tree or the maximum size of a node which is thankfully inversely related to the maximum allowed depth so in practice we only need to tune one of the two parameters. However, with $k$ trees we now have $\mathcal{O}(k)$ more parameters to tune which introduces difficulties both at the theoretical and practical level: its not clear a priori which arrangement of hyperparameters might yield better results. For lack of a clear understanding of the fourth point we leave it here as an open problem.





In a recent paper \cite{DS14} the authors propose a potential function to measure the difficulty of exact NNS. The setting is the usual one we have a query point $q \in \mathds{R}^D$ and a dataset $x_1 , \dots , x_n \in X \subseteq \mathds{R}^D$ and we'd like to find the nearest neighbor to $q$ in $X$
\[ \phi(q, \{ x_1, \dots , x_n \}) = \frac{1}{n} \sum_{i = 2}^n \frac{\| q - x_{(1)} \|}{q - x_{(i)}}  \]
Where $x_{(k)}$ denotes the $k$'th nearest neighbor of $q$. Upon further inspection of this function we can see that when its close to 1 then all the points are more or less the same distance around $q$ and we can expect nearest neighbor queries to be difficult. On the other hand, when $\phi$ is close to 0 then this means that most of the points are far away from the nearest neighbor and intuitevely we'd expect nearest neighbor to become easy. The authors determine in fact that the failure probability of an rp-tree is $\phi \log \frac{1}{\phi}$ and that of a spill tree is $\phi$. Generally though we will be considering nodes $N \subset X$ in our spatial tree so we will add a simple modification:

\[ \phi_m(q, \{ x_1, \dots , x_n \}) = \frac{1}{m} \sum_{i = k + 1}^m \frac{\| q - x_{(1)} \|}{q - x_{(i)}}  \]

 Their results easily extend to the $k$ nearest neigbhor case, a simple modification is made to the potential function $\phi$ which now becomes:

\[ \phi_{k,m}(q, \{ x_1, \dots , x_n \}) = \frac{1}{m} \sum_{i = k + 1}^m \frac{( \| q - x_{(1)} \| + \dots + \| q - x_{(k)})/k \|}{q - x_{(i)}}  \]

Finally for our contribution we first propose an extension to batch nearest neighbor by again simply modifying the potential function $\phi$ where $x_{k}^q_i$ denotes the $k$'th nearest neighbor to $q_i$

\begin{equation}

 \phi_{k,m}(\{ q_1, \dots , q_n \}, \{ x_1, \dots , x_n \}) = \frac{1}{m} \sum_{i = k + 1}^m \frac{( \| q_1 - x_{(1)}^{q_1} \| + \dots + \| q_1 - x_{(k)}^{q_1})/k \|}{q_1 - x_{(i)}^{q_1}} + \dots + \frac{1}{m} \sum_{i = k + 1}^m \frac{( \| q_n - x_{(1)}^{q_n} \| + \dots + \| q_n - x_{(k)}^{q_n})/k \|}{q_n - x_{(i)}^{q_n}} 

\end{equation}

The above expression takes into account how easy it is to find the nearest neighbors of a given a set of query points but it does not seem to exploit any structure from the query set $Q$. However, in the dual tree setting we know that the closer query points are the easier batch nearest neighbor queries become and we can represent this intuition as another potential function on the query set $Q$. Here we have two possible candidates either we can look at the average interpoint distance which trivially takes $\mathcal{O}(n^2)$ trivially to compute.

\begin{equation}

\phi(Q) = \sum_{i = 1}^n \sum_{j = i + 1}^n \frac{1}{n^2} \| q_i - q_j \|

\end{equation}

Alternatively we can use the diameter of $Q$ which again takes $\mathcal{O}(n^2)$ to compute.

\begin{equation}
\phi(Q) = \max_{q_i , q_j} \| q_i - q_j \|
\end{equation}

We now have all the components we need to rewrite a potential function for exact batch nearest neighbor search.

\begin{equation}

\phi(Q,X) = \phi(Q) \phi_{k,m}

\end{equation}

The new bound we then propose on batch nearest neighbor search via rp-trees is $\phi \log \frac{1}{\phi} |Q| \phi ( Q ) $ by a simple union argument. The $|Q|$ factor is alarming because the previous bounds had no dependence on the number of points in our dataset, but it is intuitive because if $\phi(Q)$ indicates that $Q$ is not well clumped together then we expect the complexity of our problem to increase linearly with the number of query points and should there be a structure to $Q$ our bound will reap its rewards.











==> testing/test_frontmatter.tex <==
%
%
% UCSD Doctoral Dissertation Template
% -----------------------------------
% http:\\ucsd-thesis.googlecode.com
%
%


%% REQUIRED FIELDS -- Replace with the values appropriate to you

% No symbols, formulas, superscripts, or Greek letters are allowed
% in your title.
\title{The Title Of The Dissertation}

\author{Your Name Here}
\degreeyear{2009}

% Master's Degree theses will NOT be formatted properly with this file.
\degreetitle{Doctor of Philosophy} 

\field{Mathematics}
\chair{Professor Chair Master}
% Uncomment the next line iff you have a Co-Chair
% \cochair{Professor Cochair Semimaster} 
%
% Or, uncomment the next line iff you have two equal Co-Chairs.
%\cochairs{Professor Chair Masterish}{Professor Chair Masterish}

%  The rest of the committee members  must be alphabetized by last name.
\othermembers{
Professor Humor Less\\ 
Professor Ironic Name\\
Professor Cirius Thinker\\
}
\numberofmembers{4} % |chair| + |cochair| + |othermembers|


%% START THE FRONTMATTER
%
\begin{frontmatter}

%% TITLE PAGES
%
%  This command generates the title, copyright, and signature pages.
%
\makefrontmatter 

%% DEDICATION
%
%  You have three choices here:
%    1. Use the ``dedication'' environment. 
%       Put in the text you want, and everything will be formated for 
%       you. You'll get a perfectly respectable dedication page.
%   
%
%    2. Use the ``mydedication'' environment.  If you don't like the
%       formatting of option 1, use this environment and format things
%       however you wish.
%
%    3. If you don't want a dedication, it's not required.
%
%
\begin{dedication} 
 To me. And you. Which equals us.
\end{dedication}

% You are responsible for formatting here.
\begin{mydedication} 
  \vspace{1in}
  \begin{flushleft}
    To me.
  \end{flushleft}
   
   \vspace{2in}
   \begin{center}
     And you.
   \end{center}

  \vspace{2in}
  \begin{flushright}
    Which equals us.
  \end{flushright}
\end{mydedication}



%% EPIGRAPH
%
%  The same choices that applied to the dedication apply here.
%

% The style file will position the text for you.
\begin{epigraph} 
  \emph{A careful quotation\\
  conveys brilliance.}\\
  ---Smarty Pants
\end{epigraph}

 % You position the text yourself.
\begin{myepigraph}
   \vfil
   \begin{center}
     \emph{A careful quotation\\
     conveys brilliance.}\\
     ---Smarty Pants
   \end{center}
 \end{myepigraph}


%% SETUP THE TABLE OF CONTENTS
%
\tableofcontents
\listoffigures  % Uncomment if you have any figures
\listoftables   % Uncomment if you have any tables



%% ACKNOWLEDGEMENTS
%
%  While technically optional, you probably have someone to thank.
%  Also, a paragraph acknowledging all coauthors and publishers (if
%  you have any) is required in the acknowledgements page and as the
%  last paragraph of text at the end of each respective chapter. See
%  the OGS Formatting Manual for more information.
%
\begin{acknowledgements} 
 Thanks to whoever deserves credit for Blacks Beach, Porters Pub, and
 every coffee shop in San Diego. 

 Thanks also to hottubs.
\end{acknowledgements}


%% VITA
%
%  A brief vita is required in a doctoral thesis. See the OGS
%  Formatting Manual for more information.
%
\begin{vitapage}
\begin{vita}
  \item[2002] B.~S. in Mathematics \emph{cum laude}, University of Southern North Dakota, Hoople
  \item[2002-2007] Graduate Teaching Assistant, University of California, San Diego
  \item[2007] Ph.~D. in Mathematics, University of California, San Diego 
\end{vita}
\begin{publications}
  \item Your Name, ``A Simple Proof Of The Riemann Hypothesis'', \emph{Annals of Math}, 314, 2007.
  \item Your Name, Euclid, ``There Are Lots Of Prime Numbers'', \emph{Journal of Primes}, 1, 300 B.C.
\end{publications}
\end{vitapage}


%% ABSTRACT
%
%  Doctoral dissertation abstracts should not exceed 350 words. 
%   The abstract may continue to a second page if necessary.
%
\begin{abstract}
  This dissertation will be abstract. 
\end{abstract}


\end{frontmatter}

%% START THE FRONTMATTER, THIS TIME WITH A Co-Chair
%
\title{The Title Of The Dissertation, But This Time A Really Really Really Long Title That Will Span More Than One Line.}

\chair{Professor Chair Master}
% Uncomment the next line iff you have a Co-Chair
\cochair{Professor Cochair Semimaster} 
%
% Or, uncomment the next line iff you have two equal Co-Chairs.
%\cochairs{Professor Chair Masterish}{Professor Chair Masterish}

%  The rest of the committee members  must be alphabetized by last name.
\othermembers{
Professor Humor Less\\ 
Professor Ironic Name\\
Professor Cirius Thinker\\
Professor Lateto Mydefense\\
}
\numberofmembers{5} % |chair| + |cochair| + |othermembers|
\begin{frontmatter}

%% TITLE PAGES
%
%  This command generates the title, copyright, and signature pages.
%
\makefrontmatter 

%% ABSTRACT
%
%  Doctoral dissertation abstracts should not exceed 350 words. 
%   The abstract may continue to a second page if necessary.
%
\begin{abstract}
  %This dissertation will be abstract. And confusing too.

 Five and Seven said nothing, but looked at Two. Two began in a low voice, `Why the fact is, you see, Miss, this here ought to have been a red rose-tree, and we put a white one in by mistake; and if the Queen was to find it out, we should all have our heads cut off, you know. So you see, Miss, we're doing our best, afore she comes, to--' At this moment Five, who had been anxiously looking across the garden, called out `The Queen! The Queen!' and the three gardeners instantly threw themselves flat upon their faces. There was a sound of many footsteps, and Alice looked round, eager to see the Queen.

First came ten soldiers carrying clubs; these were all shaped like the three gardeners, oblong and flat, with their hands and feet at the corners: next the ten courtiers; these were ornamented all over with diamonds, and walked two and two, as the soldiers did. After these came the royal children; there were ten of them, and the little dears came jumping merrily along hand in hand, in couples: they were all ornamented with hearts. Next came the guests, mostly Kings and Queens, and among them Alice recognised the White Rabbit: it was talking in a hurried nervous manner, smiling at everything that was said, and went by without noticing her. Then followed the Knave of Hearts, carrying the King's crown on a crimson velvet cushion; and, last of all this grand procession, came the King and Queen of Hearts.

\end{abstract}

\end{frontmatter}

